Star Formation Histories, Abundances and Kinematics of Dwarf Galaxies in the Local Group

Within the Local Universe galaxies can be studied in great detail star by star, and here we review the results of quantitative studies in nearby dwarf galaxies. The Color-Magnitude Diagram synthesis method is well established as the most accurate way to determine star formation history of galaxies back to the earliest times. This approach received a large boost from the exceptional data sets that wide field CCD imagers on the ground and the Hubble Space Telescope could provide. Spectroscopic studies using large ground based telescopes such as VLT, Magellan, Keck and HET have allowed the determination of abundances and kinematics for significant samples of stars in nearby dwarf galaxies. These studies have shown how the properties of stellar populations can vary spatially and temporally. This leads to important constraints to theories of galaxy formation and evolution. The combination of spectroscopy and imaging and what they have taught us about dwarf galaxy formation and evolution is the aim of this review.

==> our_defs.tex <==

\def\aapr{{Astron. \& Astrophys. Rev.}}
\def\nat{{ Nature }}
\def\aap{{ Astron. \& Astrophys. }}
\def\aaps{{ Astron. \& Astrophys.~Supp.}}
\def\aj{{ Astron.~J. }}
\def\apj{{ Astrophys.~J. }}
\def\araa{{ Ann. Rev. Astron. Astrophys. }}
\def\apjl{{ Astrophys.~J.~Letters }}
\def\apjs{{ Astrophys.~J.~Suppl. }}
\def\apss{{ Astrophys.~Space~Sci. }}
\def\icarus{{ Icarus }}
\def\mnras{{ MNRAS }}
\def\pasp{{ Pub. Astron. Soc. Pacific }}
\def\planss{{ Plan. Space Sci. }}
\def\physrep{{ Phys. Rep.}}
\def\bain{{ Bull.~Astron.~Inst.~Netherlands }}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$
}}}}


% 
\def\gsim{\;\lower.6ex\hbox{$\sim$}\kern-7.75pt\raise.65ex\hbox{$>$}\;}
\def\lsim{\;\lower.6ex\hbox{$\sim$}\kern-7.75pt\raise.65ex\hbox{$<$}\;}
                                     
\def\cc{\mbox{cm$^{-3}$}}
\def\tauv{\mbox{$\tau_V$}}
\def\av{\mbox{$A_V$}}
\def\ra{\mbox{$\rightarrow$}}
%                                                  units
\def\d{^\circ}
\def\h{^{\rm h}}
\def\mi{^{\rm m}}
\def\s{^{\rm s}}
\def\mum{\ts \mu{\rm m}}
\def\mm{\ts {\rm mm}}
\def\cm{\ts {\rm cm}}
\def\percm{\ts {\rm cm}^{-1}}
\def\m{\ts {\rm m}}
\def\kms{\rm{\, km \, s^{-1}}}
\def\K{\ts {\rm K}}
\def\Kkms{\ts {\rm K\ts km\ts s^{-1}}}
\def\kHz{\ts {\rm kHz}}
\def\MHz{\ts {\rm MHz}}
\def\GHz{\ts {\rm GHz}}
\def\pc{\ts {\rm pc}}
\def\kpc{\ts {\rm kpc}}
\def\Mpc{\ts {\rm Mpc}}
\def\cmsq{\ts {\rm cm^2}}
\def\pcsq{\ts {\rm pc^2}}
\def\dsq{\ts {\rm deg^2}}
\def\debye{\ts10^{-18}\ts {\rm esu}\ts {\rm cm}}
\def\swash2o{$1_{10} - 1_{01}$}             

%                                                  journals
%                                                  mathe
\let\ap=\approx
\let\ts=\thinspace

\def\an{{ Astronomische Nachrichten }}
\def\sci{{ Science }}
\def\prl{{ Phys. Rev. Lett. }}
\def\zfa{{ Zeitschrift fur Astrophysik }}
\def\ba{{ Baltic Astronomy }}
\def\rmp{{ Rev. Mod. Phys. }}
\def\rpp{{ Rep. Prog. Phys. }} 
\def\pasj{{ Pub. Astron. Soc. Japan }}
\def\pr{{ Phys. Rev. }}
\def\grg{{ Gen. Rel. Grav. }}
\def\sitz{{ Sitzungsber. K. Akad. }}

